Unraveling the Effect of Spatial Resolution and Scan Acceleration on 3D Image-Based Navigators for Respiratory Motion Tracking in Coronary MR Angiography

Purpose: To study the accuracy of motion information extracted from beat-to-beat 3D image-based navigators (3D iNAVs) collected using a variable-density cones trajectory with different combinations of spatial resolutions and scan acceleration factors. Methods: Fully sampled, breath-held 4.4 mm 3D iNAV datasets for six respiratory phases are acquired in a volunteer. Ground truth translational and nonrigid motion information is derived from these datasets. Subsequently, the motion estimates from synthesized undersampled 3D iNAVs with isotropic spatial resolutions of 4.4 mm (acceleration factor = 10.9), 5.4 mm (acceleration factor = 7.2), 6.4 mm (acceleration factor = 4.2), and 7.8 mm (acceleration factor = 2.9) are assessed against the ground truth information. The undersampled 3D iNAV configuration with the highest accuracy motion estimates in simulation is then compared with the originally proposed 4.4 mm undersampled 3D iNAV in six volunteer studies. Results: The simulations indicate that for navigators beyond certain scan acceleration factors, the accuracy of motion estimates is compromised due to errors from residual aliasing and blurring/smoothening effects following compressed sensing reconstruction. The 6.4 mm 3D iNAV achieves an acceptable spatial resolution with a small acceleration factor, resulting in the highest accuracy motion information among all assessed undersampled 3D iNAVs. Reader scores for six volunteer studies demonstrate superior coronary vessel sharpness when applying an autofocusing nonrigid correction technique using the 6.4 mm 3D iNAVs in place of 4.4 mm 3D iNAVs. Conclusion: Undersampled 6.4 mm 3D iNAVs enable motion tracking with improved accuracy relative to previously proposed undersampled 4.4 mm 3D iNAVs.

==> figs.tex <==
\begin{figure}[h]
  \centering
  \caption[]
    {The standard acquisition in bSSFP cones imaging provides maximal robustness to eddy current artifacts by acquiring readouts in a sequential manner from the south pole to the north pole. When 18 cones per cardiac cycle are acquired, the readouts collected during the first heartbeat for a sequential trajectory are shown in (A). Images obtained in this manner are free of any noticeable artifacts (B). Readouts collected in the first heartbeat when implementing phyllotaxis ordering with a Fibonacci number of 610 and with 18 cones per phyllotaxis segment are displayed in (C). This acquisition scheme results in significant image degradation (white arrows) due to eddy currents (D) for a 0.98 mm isotropic acquisition. Prescribing the Fibonacci number and number of cones per phyllotaxis segment as 89 and 126, respectively, mitigates the changes between consecutive excitations (E), while providing a more distributed coverage compared to a sequential collection pattern. The resulting image exhibits no apparent eddy current artifacts (F). 
    }
\end{figure}

\begin{figure}[h]
  \centering
  \caption[]
    {(A) A sequential acquisition of readouts results in notable gaps (black arrows) in $k$-space when the data is retrospectively binned into 4 respiratory phases. (B) Although the modified phyllotaxis ordering scheme for 0.98 mm isotropic bSSFP CMRA yields less distributed readouts in each heartbeat relative to the original phyllotaxis implementation for 1.2 mm imaging, it nevertheless provides uniform coverage when binned into different respiratory phases. The resulting pseudo-random undersampling in each phase facilitates parallel imaging and compressed sensing reconstruction techniques. 
    }
  \label{fig:theoryConv}
\end{figure}

\begin{figure}[h]
  \centering
  \caption[]
    {Reformatted MIP of the RCA following L\textsubscript{1}-ESPIRiT without motion correction (M1) and with translational correction (M2) for one volunteer study (A), one contrast-enhanced patient study (B), and one non-contrast-enhanced patient study (C). The proposed correction framework (M3) yields the sharpest depiction of the RCA compared to the other two approaches. Magnified 2D cross-sectional views of the coronary segments at regions indicated by solid white lines further demonstrate the superior performance of the proposed method. 
    }
\end{figure}

\begin{figure}[h]
  \centering
  \caption[]
    {The LCA without motion correction (M1) and with translational correction (M2) following L\textsubscript{1}-ESPIRiT for one volunteer study (A), one contrast-enhanced patient study (B), and one non-contrast-enhanced patient study (C). As seen with the RCA, the proposed method (M3) presents all regions of the LCA in an enhanced manner relative to M1 and M2. Magnified cross-sectional views of the coronary arteries at segments highlighted by solid white lines show improved depiction of the lumen of the LCA with M3.  
    }
\end{figure}

\begin{figure}[h]
  \centering
  \caption[]
    {(A) The average of both reader scores for the LCA and RCA across all six studies (one volunteer (V), two contrast-enhanced (CE) patients, three non-contrast-enhanced (NCE) patients) and all three motion correction techniques (M1 = L\textsubscript{1}-ESPIRiT without motion correction, M2 = L\textsubscript{1}-ESPIRiT with translational correction, M3 = proposed motion-resolved reconstruction framework with intraphase 3D translational correction). (B) The mean RCA and LCA reader scores for the three different correction approaches. The statistical significance of the results for reader scores was P $<$ 0.01 for both the RCA and LCA when using the two-tailed Student's t-test. 
    }
\end{figure}

\begin{figure}[h]
  \centering
  \caption*
    {Supporting Information Figure S1: Imaging data is collected with a cardiac-triggered sequence. A fat-saturation (FS) module is followed by a 3D cones sequence, where cones interleaves are acquired in groups of 18 with a temporal resolution of 99 ms during diastole. A 3D iNAV is also collected with a temporal resolution of 176 ms each heartbeat to monitor heart motion.
    }
\end{figure}

\begin{figure}[h]
  \centering
  \caption*
    {Supporting Information Figure S2: Applying a phyllotaxis readout ordering strategy with 610 as the Fibonacci number (B) results in eddy current artifacts in a stationary 0.98 mm isotropic resolution phantom scan. Implementing cones reordering with 89 as the Fibonacci number (C) yields image quality comparable to that obtained from the standard sequential collection pattern (A). This corroborates the trends seen in \textit{in vivo} experimentation.
    }
\end{figure}

\begin{figure}[h]
  \centering
  \caption*
    {Supporting Information Figure S3: Respiratory-resolved reconstructions of the end-expiration phase for different combinations of spatial ($\lambda_{1}$) and temporal ($\lambda_{2}$) regularization parameters. A large $\lambda_{2}$ introduces blurring across the motion states, while a very high value for $\lambda_{1}$ causes unwanted smoothening of the overall image. $\lambda_{1}$ = 0.001 and $\lambda_{2}$ = 0.005 provide a trade-off between noise reduction and blurring/smoothening effects.
    }
\end{figure}

\begin{figure}[h]
  \centering
  \caption*
    {Supporting Information Figure S4: 3D intraphase translational correction improves distal RCA sharpness in case 1 (non-contrast-enhanced). In case 2 (contrast-enhanced), a LCA branch is better depicted after accounting for the residual 3D translational motion in the end-expiration image. White arrows indicate regions of differences with intraphase correction. 
    }
\end{figure}

\begin{figure}[h]
  \centering
  \caption*
    {Supporting Information Figure S5: Corresponding gridding and L\textsubscript{1}-ESPIRiT outcomes for the four respiratory phases from one subject study. The noise-like aliasing artifacts resulting from the undersampling in each phase are well-suited for compressed sensing reconstructions. The displacement of the coronary vessel can be seen across the different respiratory motion states.
    }
\end{figure}

\begin{figure}[h]
  \centering
  \caption*
    {Supporting Information Video S1: Our cones imaging sequence acquires 18 readouts each heartbeat. The sequential collection pattern (top left) acquires readouts starting from the south pole at the beginning of the scan and progresses towards the north pole in $k$-space by the end of the scan. Ordering the readouts using a phyllotaxis scheme with a Fibonacci number of 610 and with the number of cones per phyllotaxis segment as 18 (top right) results in traversal from the bottom to the top of $k$-space each heartbeat. For 1.2 mm bSSFP imaging, eddy current artifacts are minimal. However, for 0.98 mm bSSFP imaging with variable-density sampling, image degradation due to eddy currents is observed because of larger changes in $k$-space location between adjacent excitations in a heartbeat. This is due to a larger $k_{max}$ for a 0.98 mm acquisition relative to a 1.2 mm acquisition. In consideration of the target higher resolution, we implement phyllotaxis with a Fibonacci number of 89 and with the number of cones per phyllotaxis segment as 126 (bottom).
    }
\end{figure}



==> figs_copy.tex <==
\newpage

FIG 1. Traditional algorithms for non-Cartesian regularized SENSE implicitly estimate a convolution with the sampling point spread function every iteration using nonuniform Fourier transforms (NUFFTs) (top row). The Toeplitz-based method computes a circular convolution over twice the image size using a transfer function represented in Cartesian coordinates (Eq. \ref{eq:Mdef_a}), which produces an identical result within the original image size provided that the object is bounded. Cropping after circular convolution eliminates the erroneous result outside the original image size (Eq. \ref{eq:Mdef_a}).

FIG 2. The reconstruction times for the gradient computation (i.e., $S_N^HWS_N$ for NUFFT and $Z^HF^{-1}MFZ$ for Toeplitz) for both CPU and GPU implementations for various undersampling rates and image matrix size factors compared to the nominal matrix size of $128 \times 128 \times 64$. NUFFT oversampling was 1.5 and the kernel width was 4.

FIG 3. Rates of speed increase for Toeplitz compared to NUFFT for the gradient computation (i.e., $S_N^HWS_N$ for NUFFT and $Z^HF^{-1}MFZ$ for Toeplitz) for both CPU and GPU implementations. The left panels show trends as the kernel width and oversampling ratio are varied, while the undersampling rate is fixed at 4 and the FOV size factor relative to the nominal FOV of $128 \times 128 \times 64$ is fixed at 1.5. The right panel shows trends as the undersampling rate and size factor are varied, while the NUFFT oversampling and kernel width are fixed to 1.5 and 6, respectively. Timings for 3D cones and radial trajectories were averaged with each other before computing the speed increases (individual trends were similar).

FIG 4. (a) In some non-Cartesian acquisitions, signal may lie outside the FOV the trajectory was designed for, which can be assessed from calibration data using an ESPIRiT eigenvalue threshold. (b) Compressed sensing reconstructions that ignored the signal outside the nominal matrix size exhibited errors that were eliminated when the optimal size was used.

FIG 5. Normalized root-mean-square-error (RMSE) and number of iterations required to converge as $\kappa$ is varied from 0 to 1. Shown below are differences from ground truth for $\kappa=\{0, 0.3, 0.6, 1\}$ in a sample slice. There is little change in error, but large changes in convergence speed, for $\kappa$ near 0. The difference images are scaled by 10 for 3D cones and 20 for 3D radial, relative to the ground truth image shown on the bottom left (similar results in other slices). 
    











